Toward Modeling Creative Processes for Algorithmic Painting

This paper proposes a framework for computational modeling of artistic painting algorithms, inspired by human creative practices. Based on examples from expert artists and from the author's own experience, the paper argues that creative processes often involve two important components: vague, high-level goals (e.g., "make a good painting"), and exploratory processes for discovering new ideas. This paper then sketches out possible computational mechanisms for imitating those elements of the painting process, including underspecified loss functions and iterative painting procedures with explicit task decompositions.

==> Computational Creativity and Underspecified Problems_arXiv/figuretex/analogytable.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ |c|c| }
\hline
 \textbf{Human activities} & \textbf{Computer algorithms} \\\hline
Steps, strategy, process  &
Algorithm, procedure \\
Goal-directed search &
Numerical optimization \\
Skill learning & Policy optimization, Reinforcement learning \\
Intrinsically-motivated exploration, creative play
& Open-ended search, curiosity-driven learning \\
Creative problem solving & Underspecified problem solving \\
\hline
\end{tabular}
\end{center}
\caption{A possible correspondence between human activities and the computational procedures discussed in this paper. The processes on the right provide models or metaphors to describe the activities on the left.
Some of these activities/processes may be complementary, nested, and/or overlapping, e.g., all computational algorithms are procedures. This is not meant to imply equivalence between human behaviors and computational models; as the famous quote by George Box goes: ``All models are wrong, but some are useful.''
\label{table}
}
\end{table*}

==> Computational Creativity and Underspecified Problems_arXiv/figuretex/painterly.tex <==
\newcommand{\pfigwidth}{1.5in}

\begin{figure}[t]
    \centering
    (a)
        \includegraphics[width=\pfigwidth]{litwinowicz-input.jpg}
    \includegraphics[width=\pfigwidth]{litwinowicz-output.jpg} \\
    (b)
    \includegraphics[width=\pfigwidth]{relax-input.jpg} 
    \includegraphics[width=\pfigwidth]{relax-output.jpg} \\
    (c)
\includegraphics[width=\pfigwidth]{snp-input.jpg}
    \includegraphics[width=\pfigwidth]{snp-output.jpg}
\caption{Existing approaches to stroke-based painterly image stylization.
   (a) A procedural method, where strokes are placed on a jittered grid, drawing color and orientations from a source image (Litwinowicz 1997). The stroke arrangement does not adapt to the source image.
   (b) An optimization method, allowing strokes to adapt to image content, but with a costly optimization process
    (Hertzmann 2001).
   (c) Optimization with differentiable rendering (Zou et al. 2021).
    \label{fig:painterly} 
    }
\end{figure}


==> Computational Creativity and Underspecified Problems_arXiv/figuretex/radcliffe.tex <==
\begin{figure*}
    \centering
\includegraphics[width=\figwidth]{radcliffe-intermediate.jpg}~~~
\includegraphics[width=\figwidth]{radcliffe.jpg}
    \caption{A digital painting of the Radcliffe Camera in Oxford, made in 2019 when I was still getting started with digital drawing tools. I started out intending to make a realistic watercolor of the building. I grew frustrated with watercolor, and decided to switch strategies midway through by adding ink strokes over the watercolor. The final picture didn't meet my initial goals at all---it's not very accurate, and it's not in the style I intended---but I'm still happy with it.
    \label{fig:radcliffe} }
\end{figure*}


==> Computational Creativity and Underspecified Problems_arXiv/figuretex/styles.tex <==
\newcommand{\stsize}{2in}
\begin{figure*}
    \centering
\includegraphics[height=\stsize]{Moka.jpg}
\includegraphics[height=\stsize]{lakeunion.jpg}
\includegraphics[height=\stsize]{Hibiki.jpg}
    \caption{Three examples of digital drawings in which the subject determined the style I ended up using. In the first, I used simulated oil paint to depict shading variations. In the second, I used solid-color strokes since  the water could be clustered into three distinct colors. In the third, I used semi-transparent, texture-less strokes to illustrate transparency and refraction. While each of these subjects could have been drawn in any of these styles,  the results would have been very different, and it would have been much more difficult to achieve a satisfying result. %
    }
    \label{fig:styles}
\end{figure*}

==> Computational Creativity and Underspecified Problems_arXiv/figuretex/sunset.tex <==
\newcommand{\sunsetwidth}{1.5in}
\begin{figure}
\centering
 \includegraphics[width=\sunsetwidth]{sunset1.JPG}
 \includegraphics[width=\sunsetwidth]{sunset2.JPG}
 \includegraphics[width=\sunsetwidth]{sunset3.JPG}
 \includegraphics[width=\sunsetwidth]{rock.JPG}
\caption{Four paintings made at roughly the same time in the same spot, illustrating how different choices of media and technique can produce very different outcomes. I painted the first three quickly en plein air, and the fourth from a photograph later on. Each one surprised me when completed.}
    \label{fig:sunset}
\end{figure}
